Towards Gravity From a Color Symmetry

Using tools from color-kinematics duality we propose a holographic construction of gravitational amplitudes, based on a 2d Kac-Moody theory on the celestial sphere. In the $N\to \infty$ limit the gauge group corresponds to $w_{1+\infty}$, due to the $U(N)$ generators enjoying a simple quantum group structure, which is in turn inherited from a twistor fiber over the celestial sphere. We show how four-dimensional momentum-space is emergent in this picture, which connects directly to the so-called kinematic algebra of the tree-level S-Matrix. On the other hand, the framework can be embedded within a celestial CFT to make contact with holographic symmetry algebras previously observed in the soft expansion. Kac-Moody currents play the role of a graviton to all orders in such expansion, and also lead to a natural notion of Goldstone modes for $w_{1+\infty}$. Focusing on MHV amplitudes, main examples are a BCFW type recursion relation and holomorphic three-point amplitudes.

==> TW2 3/author_list.tex <==
% remove these 3 lines before journal submittal.
%\centerline{author list dated 18 June 2018}
% end removal before journal submittal

\author{Alfredo Guevara } \email[]{aguevaragonzalez@fas.harvard.edu}  \affiliation{Center for the Fundamental Laws of Nature, Society of Fellows, \& Black Hole Initiative,
Harvard University, Cambridge, MA 02138, USA}
%
% visitor_addresses.tex                       18 June 2018
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
 \noaffiliation
%
\vskip 0.25cm

